Privately Estimating a Gaussian: Efficient, Robust and Optimal

In this work, we give efficient algorithms for privately estimating a Gaussian distribution in both pure and approximate differential privacy (DP) models with optimal dependence on the dimension in the sample complexity. In the pure DP setting, we give an efficient algorithm that estimates an unknown $d$-dimensional Gaussian distribution up to an arbitrary tiny total variation error using $\widetilde{O}(d^2 \log \kappa)$ samples while tolerating a constant fraction of adversarial outliers. Here, $\kappa$ is the condition number of the target covariance matrix. The sample bound matches best non-private estimators in the dependence on the dimension (up to a polylogarithmic factor). We prove a new lower bound on differentially private covariance estimation to show that the dependence on the condition number $\kappa$ in the above sample bound is also tight. Prior to our work, only identifiability results (yielding inefficient super-polynomial time algorithms) were known for the problem. In the approximate DP setting, we give an efficient algorithm to estimate an unknown Gaussian distribution up to an arbitrarily tiny total variation error using $\widetilde{O}(d^2)$ samples while tolerating a constant fraction of adversarial outliers. Prior to our work, all efficient approximate DP algorithms incurred a super-quadratic sample cost or were not outlier-robust. For the special case of mean estimation, our algorithm achieves the optimal sample complexity of $\widetilde O(d)$, improving on a $\widetilde O(d^{1.5})$ bound from prior work. Our pure DP algorithm relies on a recursive private preconditioning subroutine that utilizes the recent work on private mean estimation [Hopkins et al., 2022]. Our approximate DP algorithms are based on a substantial upgrade of the method of stabilizing convex relaxations introduced in [Kothari et al., 2022].

==> sec/alt-analysis-gaussian-sampling.tex <==
% \section{Alternative Analysis of the Gaussian Sampling Mechanism}\label{sec:alt-analysis}
% In this section, we provide an alternative analysis of the Gaussian Sampling Mechanism (Algorithm \ref{alg:cov-noise-mechanism}). We note, however, that this analysis requires a stronger sensitivity bound $\Delta$ on the algorithm $\mathcal{M}$ than \cref{thm:gaussian-sampling-mech}.

% Given recent work (e.g.,~\cite{AZ22}) showing the characterizations of
% local DP mechanisms via the
% contraction coefficient of $f$-divergences, we believe
% Theorem~\ref{thm:gaussian-sampling-mech-alt} could be useful for other
% DP mechanisms.

% \begin{theorem}[Alternative Analysis of the Gaussian Sampling Mechanism via Hockey-Stick Divergence Bound]
% \label{thm:gaussian-sampling-mech-alt}
% Fix $\varepsilon, \delta \in (0, 1)$ and $k \in \mathbb{N}$.
% Let $C$ be an absolute constant and  \[\Delta \leq \frac{1}{C} \min \left(1, \frac{\epsilon}{4\sqrt{kd} \log(1/\delta)}\right).\]
% Let $\mathcal{M}: \left(\R^{d}\right)^n \rightarrow \mathbb{S}_+^d$ be a (randomized) algorithm that given a dataset of $n$ points in $\mathbb{R}^d$ outputs a PSD matrix. 
% Suppose that $\mathcal{M}$ satisfies a sensitivity bound  that \[\left\|\mathcal M({\cal Y})^{1/2}\mathcal M({\cal Y}')^{-1}\mathcal M({\cal Y})^{1/2} - I\right\|_F \le \Delta\] for any neighboring datasets  $\mathcal{Y}, \mathcal{Y}'$. Then given an input $\Sigma = \mathcal{M}(\mathcal{Y})$, 
% \begin{itemize}
%     \item Algorithm \ref{alg:cov-noise-mechanism} is $(\varepsilon, \delta)$-DP (with respect to the original dataset $\mathcal{Y}$); and
%     \item  Algorithm \ref{alg:cov-noise-mechanism} satisfies the following utility guarantee with probability $1-\gamma$:\[(1-\rho) \Sigma \preceq \widehat{\Sigma} \preceq (1+\rho) \Sigma,\]
% for $\rho = O \left(\sqrt{\frac{d + \log(1/\gamma)}{k}} + \frac{d + \log(1/\gamma)}{k} \right)$, where $\widehat{\Sigma}$ is its output.
% \end{itemize}
% \end{theorem}
% \begin{proof}
% It suffices to show that Algorithm~\ref{alg:cov-noise-mechanism} is $(\epsilon', \delta')$-DP when $k=1$ provided that $\Delta \leq \epsilon'/C\sqrt{d}$ and $d \geq C \log^2(1/\delta')$. For general $k$, we then apply~\cref{thm:adv-comp} for the $k$-fold composition with $\epsilon' = \epsilon/ 4 \sqrt{k} \log(1/\delta)$ and $\delta' = \delta / 2k$ to conclude that Algorithm~\ref{alg:cov-noise-mechanism} is $(\epsilon, \delta)$-DP. For $k=1$, by~\cref{fact:hockeystick-to-dp}, it remains to show that 
% \[
% D_{e^{\epsilon'}} (\calN(0, \Sigma), \calN(0, \Sigma')) \leq \delta',
% \]
% where $\Sigma, \Sigma'$ satisfy $\norm{\Sigma^{1/2} (\Sigma')^{-1} \Sigma^{1/2} - I}_F \leq \Delta$. This follows directly from the hypotheses and \cref{lemma:gaussian-divergence}. Finally, the utility guarantee is immediately implied by~\cref{thm:emp-cov-concentration}.
% \end{proof}




% \begin{lemma}[Hockey-stick divergence bound]
% \label{lemma:gaussian-divergence}
% Let $\Sigma_1, \Sigma_2 \in \R^{d \times d}$ be PSD matrices and $\Delta \geq 0$. There is a constant $c$ such that if $\norm{\Sigma_2^{1/2} \Sigma_1^{-1} \Sigma_2^{1/2} - I}_F \leq \Delta$ and $\Delta \leq 2c/9$, then  \[D_{\gamma}(\calN(0,\Sigma_1), \calN(0, \Sigma_2)) \leq 2 \gamma \exp\left(-4c \sqrt{d}\right) + 2 \exp \left(-\sqrt{d}/2\right)\] for any $\gamma \geq \exp(3\Delta \sqrt{d})$.
% \end{lemma}
% \begin{proof}
% Let $M = \Sigma_2^{-1/2} \Sigma_1 \Sigma_2^{-1/2}$ and the densities of $\calN(0,M), \calN(0,I)$ be $p,q$, respectively. We may directly compute the hockey-stick divergence as: 
% \begin{align*}
% D_\gamma (\calN(0,\Sigma_1), \calN(0, \Sigma_2)) &= D_\gamma (\calN(0,I), \calN(0, M))\\
% &= \int_{x \in \reals^d} [p(x) - \gamma q(x)]_+ dx \\
% &= \int q(x) \left[\frac{p(x)}{q(x)} - \gamma\right]_+ dx \\
% &= \E_{g \sim \calN(0,I)} \left[p(g)/q(g) - \gamma\right]_+ \\
% &= \E_g \left[ \sqrt{\frac{\det(I)}{\det (M)}} \exp(-g^T(M^{-1} - I)g/2) - \gamma \right]_+ \\
% &= \E_g \left[ \sqrt{\det (M^{-1})} \exp(-g^T(M^{-1} - I)g/2) - \gamma \right]_+.
% \end{align*}
% Now, note that the determinant is upper-bounded as follows:
% \[
% \log \det (M^{-1}) \leq \Tr (M^{-1} - I) \leq \sqrt{d} \norm{M^{-1} - I}_F \leq \sqrt{d} \Delta.
% \]
% Defining $A = I - M^{-1}$ and $Z = g^T A g$ and using the previous inequality, we have that the hockey-stick divergence $D_\gamma (\calN(0,\Sigma_1), \calN(0, \Sigma_2))$ is upper bounded by:
% \begin{align*}
% &\E_g \left[ \exp(\Delta \sqrt{d}/2) \exp(Z/2) - \gamma \right]_+ \\
% &= \int_{0}^\infty \Pr \left(\left[e^{(\Delta \sqrt{d} + Z)/2} - \gamma\right]_+ \geq t\right) \mathrm{d}t \\
% &\leq \int_{0}^\infty \Pr \left(e^{(\Delta \sqrt{d} + Z)/2} - \gamma \geq t\right) \mathrm{d}t \\
% &= \int_{0}^\infty \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) \mathrm{d}t \\
% &= \int_{0}^\gamma \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) \mathrm{d}t + \int_{\gamma}^\infty \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) \mathrm{d}t \\
% &\leq \gamma \Pr \left(Z \geq 2\log (\gamma) - \Delta \sqrt{d}\right) + \int_{\gamma}^\infty \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) \mathrm{d}t \\
% &\leq \gamma \Pr \left(Z \geq 5 \Delta \sqrt{d}\right) + \int_{\gamma}^\infty \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right)\mathrm{d}t. 
% \end{align*}
% We now control the two tail probabilities separately. To bound $\Pr \left(Z \geq 5 \Delta \sqrt{d}\right)$, note that \[\E Z = \Tr (A) \leq \sqrt{d} \norm{A}_F \leq \Delta \sqrt{d}.\] It follows that \[\Pr \left(Z \geq 5 \Delta \sqrt{d}\right) \leq \Pr \left(|Z -\E Z| \geq 4\Delta \sqrt{d}\right).\] By the Hanson-Wright inequality (\cref{thm:hanson-wright}), we have that, for some absolute constant $c > 0$,
% \begin{align*}
% \Pr \left(|Z -\E Z| \geq 4\Delta \sqrt{d}\right) &\leq 2\exp \left(-c \min \left ( \frac{16 \Delta^2 d}{\norm{A}_F^2}, \frac{4 \Delta \sqrt{d}}{\norm{A}_2}\right )\right)  \\
% &\leq 2\exp \left(-c \min \left ( 16d, 4 \sqrt{d} \right )\right) \\
% &= 2\exp\left(-4c \sqrt{d}\right).
% \end{align*}
% For the other tail probability, when $t \geq \gamma$, it holds that
% \begin{align*}
% \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) &\leq  \Pr \left(Z \geq 2\log(t) - \Delta \sqrt{d}\right) \\
% &\leq \Pr \left(|Z - \E Z| \geq 2\log(t) - 2\Delta \sqrt{d}\right) \\
% &\leq  \Pr \left(|Z - \E Z| \geq 4 \log(t)/ 3\right) \\
% &\leq 2\exp \left(-c \min \left( \frac{16 \log^2 (t)}{9 \Delta^2}, \frac{4 \log(t)}{3 \Delta} \right) \right) \\
% &= 2\exp \left(- 4c \log(t)/3 \Delta \right).
% \end{align*}
% Next, assuming that $\Delta \leq c_0 = 2c/9$, we can bound the integral above as
% \begin{align*}
% \int_{\gamma}^\infty \Pr \left(Z \geq 2\log(t + \gamma) - \Delta \sqrt{d}\right) \mathrm{d}t &\leq 2 \int_{\gamma}^\infty \exp \left(- 4c \log(t)/3 \Delta \right) \mathrm{d}t \\
% &= 2 \int_{\gamma}^\infty t^{- 4c /3 \Delta} \mathrm{d}t \\
% &= \frac{2}{(4c/3 \Delta - 1) \gamma^{4c/3 \Delta - 1}} \\
% &\leq 2 \exp (-\sqrt{d}/2).
% \end{align*}
% Assembling these bounds, we have that 
% \[
% D_\gamma \left(\calN(0,\Sigma_1), \calN(0, \Sigma_2)\right) \leq 2 \gamma \exp\left(-4c \sqrt{d}\right) + 2 \exp \left(-\sqrt{d}/2\right),
% \]
% which completes the proof.
% \end{proof}

